TAP-Net: Transport-and-Pack using Reinforcement Learning

We introduce the transport-and-pack(TAP) problem, a frequently encountered instance of real-world packing, and develop a neural optimization solution based on reinforcement learning. Given an initial spatial configuration of boxes, we seek an efficient method to iteratively transport and pack the boxes compactly into a target container. Due to obstruction and accessibility constraints, our problem has to add a new search dimension, i.e., finding an optimal transport sequence, to the already immense search space for packing alone. Using a learning-based approach, a trained network can learn and encode solution patterns to guide the solution of new problem instances instead of executing an expensive online search. In our work, we represent the transport constraints using a precedence graph and train a neural network, coined TAP-Net, using reinforcement learning to reward efficient and stable packing. The network is built on an encoder-decoder architecture, where the encoder employs convolution layers to encode the box geometry and precedence graph and the decoder is a recurrent neural network (RNN) which inputs the current encoder output, as well as the current box packing state of the target container, and outputs the next box to pack, as well as its orientation. We train our network on randomly generated initial box configurations, without supervision, via policy gradients to learn optimal TAP policies to maximize packing efficiency and stability. We demonstrate the performance of TAP-Net on a variety of examples, evaluating the network through ablation studies and comparisons to baselines and alternative network designs. We also show that our network generalizes well to larger problem instances, when trained on small-sized inputs.

==> figures/pack.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/packing3.pdf}
\caption{
\rh{Maximal-Connected-Space packing strategy. All the candidate positions for placing object $C$ with object $A$ and $B$ packed already are found by locating all the corner locations (first four candiates) as well as connecting location of different packed objects (last candidate) at different layers, with the remaning usable space afterward highlighed by light blue color. 
(filled with light blue color).  
The candidate location that yields the maximum remaining usable space as well as maximal packing reward is chosen and indicated using the red box.}
\rhc{Maybe we should give the strategy another name since the final space we found are actually not connected, take the first packing state as en example... } }
\label{fig:pack}
\end{figure}


==> figures/tab_comp_10_times.tex <==
\begin{table}[!t]%
	\caption{\cb{Performance of \tapnet{} trained and tested on the same datasets but multiplied by 10. [name of the table need to change]}}
	\label{tab:comp_10_times}
	\begin{minipage}{\columnwidth}
		\begin{center}
		%	\begin{tabular}{p{2.4cm}|r|r|r|r}
		\begin{tabular}{l||l||l|l|l|l}
            \hline\hline
			\textbf{Data} & \textbf{Resolution} & $C$ & $P$ & $S$ & $R$ \\ \hline \hline 
			
			\multirow{2}{*}{\emph{RAND}} 
            & \emph{Low}  & 0.925 & 0.988 & 0.997 & 0.970 \\ \cline{2-6} 
            & \emph{High} & 0.896 & 0.981 & 0.991 & 0.956 \\ \hline \hline 
			
            \multirow{2}{*}{\emph{PPSG}} 
			& \emph{Low}  & 0.981 & 0.996 & 0.999 & 0.992 \\ \cline{2-6} 
			& \emph{High} & 0.981 & 0.996 & 0.998 & 0.992 \\ \hline \hline

		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_comp_baseline_.tex <==
\begin{table}[!t]%
	\caption{Performance comparison between \tapnet{} and the two baseline \rh{ordering} algorithms on both RAND and PPSG datasets.} %\mlc{change baseline to Random and Search to Greedy in all tables.}}
	\label{tab:comp_baseline}
	\begin{minipage}{\columnwidth}
		\begin{center}
		%	\begin{tabular}{p{2.4cm}|r|r|r|r}
		\begin{tabular}{l||l||l|l|l|l|l}
			\hline\hline
			\textbf{Data} & \textbf{Method} & $C$ & $P$ & $S$ & $R$ & $t(ms)$ \\ \hline \hline 
			
%			\multirow{3}{*}{\emph{RAND}} 
%			& \rh{Random} & 0.732 & 0.895 & 0.941 & 0.856 &  5 \\ \cline{2-7} 
%			& \rh{Greedy} & 0.816 & 0.972 & 0.977 & 0.922 & 20 \\ \cline{2-7} 
%			& \textbf{\tapnet{}} & \textbf{0.925} & \textbf{0.988} & \textbf{0.997} & \textbf{0.970} & \textbf{3} \\ \hline \hline 
			
			\multirow{3}{*}{\emph{PPSG}} 
			& \rh{Random}  & 0.771 & 0.849 & 0.911 & 0.843 &  8 \\ \cline{2-7} % MACS
			& \rh{Greedy}  & 0.920 & 0.971 & 0.990 & 0.960 & 45 \\ \cline{2-7} % MACS
			& \textbf{\tapnet{}} & \textbf{0.981} & \textbf{0.996} & \textbf{0.999} & \textbf{0.992} & \textbf{3} \\ \hline \hline 
%			\multirow{3}{*}{\emph{MIX}} & Rand-Base & 0.000 & 0.000 &  0.000 &  0.000   \\ \cline{2-6} 
%			& Max-Base & 0.000 & 0.000 &  0.000 &  0.000   \\ \cline{2-6} 
%			& \textbf{Ours} & \textbf{0.000}    & \textbf{0.000} & \textbf{0.000}  & \textbf{0.000} \\ \hline \hline 
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_comp_heightmap_3D.tex <==
\begin{table}[!t]%
	\caption{C,P,S scores of the network on 3D with/without heightmap.}
	\label{tab:comp_heightmap_3D}
	\begin{minipage}{\columnwidth}
		\begin{center}
		%	\begin{tabular}{p{2.4cm}|r|r|r|r}
		\begin{tabular}{l||l||l|l|l|l}
			\hline\hline
			\textbf{Data} & \textbf{Method} &  $C$ & $P$&  $S$  &  $R$  \\ \hline \hline
			\multirow{3}{*}{\emph{RAND}} & Shape only &0.000 & 0.000 &  0.000 &  0.000  \\ \cline{2-6} 
			& Heightmap only & 0.000 & 0.000 &  0.000 &  0.000 \\  \cline{2-6} 
			& \textbf{Both} & \textbf{0.000}    & \textbf{0.000} & \textbf{0.000}  & \textbf{0.000}   \\  \hline \hline
			\multirow{3}{*}{\emph{GT}} & Shape only& 0.000 & 0.000 &  0.000 &  0.000   \\ \cline{2-6} 
			& Heightmap only&0.000 & 0.000 &  0.000 &  0.000   \\  \cline{2-6} 
			& \textbf{Both} & \textbf{0.000}    & \textbf{0.000} & \textbf{0.000}  & \textbf{0.000} \\ \hline \hline
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_comp_high_reso.tex <==
\begin{table}[!t]%
	\caption{\cb{Performance comparison between \tapnet{} and the two baseline algorithms on both RAND and PPSG datasets in 10-times resolution.}}
	\label{tab:comp_high_reso}
	\begin{minipage}{\columnwidth}
		\begin{center}
		%	\begin{tabular}{p{2.4cm}|r|r|r|r}
		\begin{tabular}{l||l||l|l|l|l|l}
			
            \hline\hline
			\textbf{Data} & \textbf{Method} & $C$ & $P$ & $S$ & $R$ & $t(ms)$ \\ \hline \hline 
			\multirow{3}{*}{\emph{RAND}}
            & Baseline & 0.620 & 0.880 & 0.972 & 0.824 & 18 \\ \cline{2-7} 
			& Search   & 0.702 & \textbf{0.951} & \textbf{0.989} & 0.881 & 58 \\ \cline{2-7} 
			& \textbf{\tapnet{}} & \textbf{0.785} & 0.946 & 0.980 & \textbf{0.904} & \textbf{4} \\ \hline \hline 
			
            \multirow{3}{*}{\emph{PPSG}}
            & Baseline & 0.669 & 0.856 & 0.956 & 0.827 & 17 \\ \cline{2-7} 
			& Search   & 0.783 & 0.952 & \textbf{0.990} & 0.908 & 56  \\ \cline{2-7} 
			& \textbf{\tapnet{}} & \textbf{0.847} & \textbf{0.956} & 0.982 & \textbf{0.928} & \textbf{4} \\ \hline \hline

		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_comp_packing.tex <==
\begin{table}[!t]%
	\caption{\mlc{merge this table into next one}}
	\label{tab:comp_packing_to_be_removed}
	\begin{minipage}{\columnwidth}
		\begin{center}
		%	\begin{tabular}{p{2.4cm}|r|r|r|r}
		\begin{tabular}{c||l|l|l|l}
			\hline
			\textbf{Packing Method} &  $C$ & $P$&  $S$  &  $R$ \\ \hline
			% \textbf{10} & \textbf{0.910 } & \textbf{0.984} & \textbf{0.990} & \textbf{0.961} \\ \hline
			LB  & 0.739 & 0.889 & 0.935 & 0.854 \\ \hline
			MUL & 0.734 & 0.895 & \textbf{0.947} & 0.859 \\ \hline
			MACS & \textbf{0.746} & \textbf{0.897} & 0.941 & \textbf{0.861} \\ \hline
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/train_ex.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{images/train_ex.png}
\caption{\rz{Our trained network generates optimal packings that are different from training examples. To generate the training pair, we {\em randomly\/}
     partition a large box that fills the target container into a set of smaller boxes and randomly arrange the resulting boxes into the initial box configuration.}}
\label{fig:train_ex}
\end{figure}

